Half-Moon Cookie: Private, Similarity-Based Blocklisting with TOCTOU-Attack Resilience

Blocklisting is a common technique for preventing the use of known malicious content. However, conventional blocklisting infrastructures require either the blocklist to be public or clients to reveal their queries to the blocklist server. We introduce a private blocklisting framework, Half-Moon Cookie, by which a client can check an item against a proprietary blocklist held by a server, to determine whether the item is close to any blocklist element in a metric space. Critically, our design separates the embedding step from the blocklist check, enabling independent choice of methods to compute them privately and efficiently. Still, this computation might be too costly to perform on the critical path of using the item, and so our design also supports a very efficient check that an item previously passed the blocklist check. In doing so, we support applications where one client can perform the blocklist check on the item before sending it, and recipients can more efficiently confirm the previous result before using the item, thereby avoiding TOCTOU attacks. We show how Half-Moon Cookie can be instantiated for similarity-based malware detection, to block malicious executables without revealing client inputs or disclosing the blocklist.

==> figure/EC.tex <==
\begin{tikzpicture}[scale=0.9]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mygray1}{RGB}{96,96,96}
\definecolor{mygray2}{RGB}{128,128,128}
\definecolor{mygray3}{RGB}{169,169,169}

\begin{groupplot}[group style={group size=4 by 1, horizontal sep=1.5cm}, height=5cm, width=\textwidth]
\nextgroupplot[
title={A},
legend cell align={left},
legend style={
	fill opacity=0.8,
	draw opacity=1,
	text opacity=1,
	at={(0.03,0.97)},
	anchor=north west,
	draw=lightgray204,
	font=\small,
},
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
%xmin=-200, xmax=10300,
xtick style={color=black},
xlabel={\server Workload},
%xticklabels={$0$,$0$, $200$, $400$}, 
%ymin=-0.5,
ymax=1100,
y grid style={darkgray176},
ylabel={$\client[1]$ Latency (s)},
ylabel style={yshift=-1ex},
%ymin=-1, ymax=20,
ytick style={color=black},
height=4.5cm,
width=4cm,
%xshift=0.1cm,
]
\addplot [semithick, black]
table {%
1 19.11
3 19.38
5 19.62
10 21.08
20 27.08
40 28.92
50 37.5
60 41.99
70 47.76
80 55.96
100 62.49
150 94.01
200 121.69
250 187.65
300 487.07
400 935.43
};
\addplot [semithick, dashed, black]
table {%
1 75.84
3 81.25
5 83.13
10 92.8
20 94.68
30 98.09
40 109.64
50 129.63
80  285.49
100 695.42
120 1374.44
};
\addplot [semithick, dotted, black]
table {%
1 786.12
3 818.9
5 846.26
10 1058.94
20 1676.73
};
\addplot [semithick, red]
table {%
1 247.04
3 253.02
5 257.2
10 350.3
20 608.78
30 1796.5
};
\nextgroupplot[
title={B},
legend cell align={left},
legend style={
	fill opacity=0.8,
	draw opacity=1,
	text opacity=1,
	at={(0.03,0.97)},
	anchor=north west,
	draw=lightgray204,
	font=\small,
},
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
%xmin=-200, xmax=10300,
xtick style={color=black},
xlabel={\server Workload},
xticklabels={$0$,$0$, $200$, $400$}, 
%ymin=-0.5,
ymax=1100,
y grid style={darkgray176},
ylabel={$\client[1]$ Latency (s)},
ylabel style={yshift=-1ex},
%ymin=-1, ymax=20,
ytick style={color=black},
height=4.5cm,
width=4cm,
%xshift=0.1cm,
]
\addplot [semithick, black]
table {%
1 19.11
3 19.38
5 19.62
10 21.08
20 27.08
40 28.92
50 37.5
60 41.99
70 47.76
80 55.96
100 62.49
150 94.01
200 121.69
250 187.65
300 487.07
400 935.43
};
\addplot [semithick, dashed, black]
table {%
1 109.14
3 109.41
5 109.65
10 111.11
20 117.11
40 118.95
50 127.53
60 132.02
70 137.79
80 145.99
100 152.52
150 184.04
200 211.72
250 277.68
300 577.1
400 1025.46
};
\addplot [semithick, dotted, black]
table {%
1 211.26
3 211.52
5 211.77
10 213.32
20 219.32
40 221.06
50 231.74
60 234.23
70 240
80 247.3
100 254.74
150 286.25
200 313.93
250 379.89
300 679.31
400 1127.67
};
\addplot [semithick, red]
table {%
1 247.04
3 253.02
5 257.2
10 350.3
20 608.78
30 1796.5
};
\end{groupplot}

\end{tikzpicture}
